Local Boosting for Weakly-Supervised Learning

Boosting is a commonly used technique to enhance the performance of a set of base models by combining them into a strong ensemble model. Though widely adopted, boosting is typically used in supervised learning where the data is labeled accurately. However, in weakly supervised learning, where most of the data is labeled through weak and noisy sources, it remains nontrivial to design effective boosting approaches. In this work, we show that the standard implementation of the convex combination of base learners can hardly work due to the presence of noisy labels. Instead, we propose $\textit{LocalBoost}$, a novel framework for weakly-supervised boosting. LocalBoost iteratively boosts the ensemble model from two dimensions, i.e., intra-source and inter-source. The intra-source boosting introduces locality to the base learners and enables each base learner to focus on a particular feature regime by training new base learners on granularity-varying error regions. For the inter-source boosting, we leverage a conditional function to indicate the weak source where the sample is more likely to appear. To account for the weak labels, we further design an estimate-then-modify approach to compute the model weights. Experiments on seven datasets show that our method significantly outperforms vanilla boosting methods and other weakly-supervised methods.

==> table/cpt_rule.tex <==
{
\begin{tabular}{ccccc}\hline
     Dataset & Anchor Category & Rec. Category & Rule Example 1 & Rule Example 2\\\hline
     Lighting & Lighting Fixture & Light Bulbs & Compatible Bulb Type = Lighting Technology &Maximum Bulb Wattage >= Wattage  \\
     Appliance & Refrigerator & Water Filter & Walter Filter Replacement Model\# = Model\# & Brand Name = Brand Compatibility\\
     Bathroom& Vanities & Faucets& Color Family = Color Family & Faucet Not Included \\
     Tools& Power Tools & Batteries& Battery Power Type = Battery Power Type & Voltage <= Voltage\\\hline
\end{tabular}
}
